Simultaneous Action Recognition and Human Whole-Body Motion and Dynamics Prediction from Wearable Sensors

This paper presents a novel approach to solve simultaneously the problems of human activity recognition and whole-body motion and dynamics prediction for real-time applications. Starting from the dynamics of human motion and motor system theory, the notion of mixture of experts from deep learning has been extended to address this problem. In the proposed approach, experts are modelled as a sequence-to-sequence recurrent neural networks (RNN) architecture. Experiments show the results of 66-DoF real-world human motion prediction and action recognition during different tasks like walking and rotating. The code associated with this paper is available at: \url{github.com/ami-iit/paper_darvish_2022_humanoids_action-kindyn-predicition}

==> sections/4-ProblemStatement.tex <==
\section{Problem Statement}
\label{sec:problemStatement}
Following the description of human motion generation and dynamics, here we try to formalize concretely the problems of human action and motion prediction. 
In this regard, first human dynamics and optimal control problem are discretized.

By discretizing \eqref{eq:state-space} and considering the optimal joint torques obtained from \eqref{eq:optimal-joint-torque}, we can write it as:
\begin{equation}
      {\bm{x}}_{k+1}^\ast = \mathcal{F}(\bm{x}_k, \bm{f}^{c}_k, \bm{\tau}^\ast_k) \Delta{t} +{\bm{x}}_k,
    \label{eq:state-space-discretized}
\end{equation}
where $\Delta{t}$ is the discretization time step.
Moreover, by discretizing \eqref{eq:optimal-joint-torque} and taking advantage of the recursive relationship between the current and previous joint torques, one can compute the optimal joint torques generated at each step by:
\begin{equation}
\begin{aligned}
\bm{\tau}_k^\ast= \mathcal{G}^\ast(\bm{x}_k, \bm{x}_{k-1}, \bm{x}_{k-2}, \dots, \bm{x}_{k-N}, \\ \bm{f}^{c}_k, \dots, \bm{f}^{c}_{k-N}, \bm{r}_k, \dots, \bm{r}_{k-N}).
\end{aligned}
\label{eq:optimal-joint-torque-discretized}
\end{equation}
In this formula, $\mathcal{G}^\ast$ is an unknown and optimal mapping with regard to \eqref{eq:optimal-joint-torque}, $N$ is the number of time steps to look behind in time.
Finally, replacing $ \bm{\tau}^\ast_k$ in \eqref{eq:state-space-discretized} with  \eqref{eq:optimal-joint-torque-discretized}, we can derive the following nonlinear optimal formulation:
%%%%%%%%%%%
\begin{equation}
\begin{aligned}
    {\bm{x}}_{k+1}^\ast = \mathcal{H}^\ast(\bm{x}_k, \bm{x}_{k-1}, \bm{x}_{k-2}, \dots, \bm{x}_{k-N}, \\ \bm{f}^{c}_k, \dots, \bm{f}^{c}_{k-N}, \bm{r}_k, \dots, \bm{r}_{k-N}),
    \end{aligned}
    \label{eq:optimal-state-space-discretized}
\end{equation}
% where $\Delta{t}$ is the discretization time step.
where $\mathcal{H}^\ast$ is an unknown optimal nonlinear function, mapping the input terms to the next state vector $\bm{x}_{k+1}^\ast$.
In this formula, the input terms $\bm{x}_{k-i}$, $\bm{f}^{c}_{k-i}$, and $\bm{r}_{k-i}$ are the states of the system, the vector of external wrenches acting on the human body, and the vector of hidden states at $i$-steps in the past.
% that affect the generated joint torques.

%%%%%%%%%%%
% \textcolor{blue}{
% \item [$\bm{f}^{c}_{k-i}$] it is the vector of external wrenches acting on the human body at $i$-step before,
% \item [$\bm{r}_{k-i}$] it is a vector of hidden states that affects the generated joint torques at $i$-step before.
% }

% \textcolor{blue}{
% Finally, replacing \eqref{eq:optimal-joint-torque-discretized} with $\bm{\tau}^\ast_k$ in \eqref{eq:optimal-state-space-discretized}, we can derive the following nonlinear optimal formulation for :
% Now, let's explain in more detail the terms inside the mapping $\mathcal{H}^\ast$:
% \begin{itemize}
%     \item [$x_{k-i}$] it is the state of the system at $i$-step before, 
%     \item [$\bm{f}^{c}_{k-i}$] it is the vector of external wrenches acting on the human body at $i$-step before,
%     \item [$\bm{r}_{k-i}$] it is a vector of hidden states that affects the generated joint torques at $i$-step before.
% \end{itemize}
% }
%%%%%%%%%%%%%%%%%%%%%
% By recursively applying \eqref{eq:optimal-state-space-discretized}, we can predict the future states of the human dynamical system for the time horizon $T$, i.e., $\bm{x}_{k+1}^\ast, \bm{x}_{k+2}^\ast, \dots, \bm{x}_{k+T}^\ast$. However, to estimate the future states of the human system in a recursive fashion, there are the following problems that needs to be addressed: ${i})$ the mapping $\mathcal{H}^\ast$ in \ref{eq:optimal-state-space-discretized} \textit{is not known}; ${ii})$ external forces/torques acting on the human in the future $ \bm{f}^{c}_{k+i}$ in \ref{eq:optimal-state-space-discretized} \textit{are not known};
% ${iii})$ the hidden states  $\bm{r}_{k\pm i}$ are not known in \ref{eq:optimal-state-space-discretized}, neither in the past nor the future.
% In the next section, we propose our solution in order to solve these problems associated with the human motion prediction.


By recursively applying \eqref{eq:optimal-state-space-discretized}, we can predict the future states of the human dynamical system for the time horizon $T$, i.e., $\bm{x}_{k+1}^\ast, \bm{x}_{k+2}^\ast, \dots, \bm{x}_{k+T}^\ast$. However, to estimate the future states of the human system in a recursive fashion, there are the following problems that needs to be addressed: ${i})$ the mapping $\mathcal{H}^\ast$ in \eqref{eq:optimal-state-space-discretized} is unknown;
% \textbf{AT THIS POINT, THE READER THAT DOES NOT READ THE APPENDIX WONDERS: SO WHY DID YOU SHOW THAT THE APPENDIX THE DERIVATION?} --> H* cannot be learned becuase we do not have all the inputs.
${ii})$ external forces/torques acting on the human in the future $ \bm{f}^{c}_{k+i}$ in \eqref{eq:optimal-state-space-discretized} are not known;
${iii})$ the hidden states  $\bm{r}_{k\pm i}$ in \eqref{eq:optimal-state-space-discretized} are not known, neither in the past nor the future.
% In the next section, we propose our solution in order to solve these problems associated with the human motion prediction.


% In order to predict human motion, we learn from human demonstrations for relevant tasks. More specifically, for the identified problems, we address them as follows.
% To address these derived challenges for human motion prediction, we propose a learning-based approach, i.e., 
% the mapping $\mathcal{H}^\ast$ in \eqref{eq:optimal-state-space-discretized} is learned from human demonstrations.
% In the literature, approaches based on a single neural network have been proposed to learn the mapping $\mathcal{H}^\ast$. 
% However, $\mathcal{H}^\ast$ is very complex, and yet no approach has resolved this problem effectively.
% and efficiently for real-time applications.


==> sections/proposedSolution.tex <==
\section{Possible Architectures for Human Action and Motion Prediction }
\label{sec:appendix:Architectures}

\begin{figure}
\centering
\begin{subfigure}[b]{0.43\textwidth}
\includegraphics[width=\textwidth]{figures/MoeArchitectures.png}
\caption{}
\label{fig:MoE:architecture}
\end{subfigure}
~
\begin{subfigure}[b]{0.53\textwidth}
\includegraphics[width=\textwidth]{figures/OtherArchitectures.png}
\caption{}
\label{fig:other_architectures}
\end{subfigure}
\caption{Schematic of possible architectures for human action and motion prediction based on supervised learning techniques. a) proposed architecture based on MoE, b) proposed architectures in the literature for human action and motion prediction.}
\label{fig:design_architectures}
\end{figure}

Following the related work in the literature to solve simultaneously the problem of action and motion prediction, Fig.~\ref{fig:design_architectures} indicates different design choices and architectures relying on supervised learning techniques.
An approach is to solve the two problems separately and in parallel, as shown in Fig.~\ref{fig:other_architectures} on top. 
However, this design choice neglects the correlation and the inherent interconnection of the two problems.
This approach introduces the risk that the predicted action and motion do not coincide, i.e., the action $a_i$ is recognized while the predicted motion is related to action $a_j$. Moreover, the proposed approach may hardly generalize to various motions and actions, especially if they are similar.
To overcome the first discussed problem and correlate the action and motion prediction together, one may devise first to predict the human action and provide as input (along with other inputs) to the motion prediction problem, as shown in Fig.~\ref{fig:other_architectures} in the middle. 
However, action prediction results influence the motion prediction, but not reversely; moreover, the two problems are trained separately.
Moreover, this design choice may suffer when generalizing over various actions.
Following that, Fig.~\ref{fig:other_architectures} in the bottom shows an architecture where a single network recognizes human action, and a pool of networks predicts human motion, picked up by a selector, similar to the idea MoE.
A choice for the selector is to choose the network associated with the recognized action, i.e., the highest probability. According to this formulation, the problems of action and motion prediction are partially interconnected, and the networks are learned separately in the training phase. However the result of action recognition affects the result of motion prediction in the online phase, the action recognition network is trained independently from the motion prediction.
This approach solves the problem of generalization over different actions; nevertheless, it introduces a discontinuity problem during the transient phases when human switches from an action to another. To overcome this, one may consider using a weighted summation of motion prediction over different action probabilities.
% - In the literature, an approach is to solve the two problems separately 
% - Another approach is to solve action recognition first and then solve the problem of motion prediction using a single NN. 

% - These approaches suffers from poor performance when generalizing over various human actions.

% - Similarly, we can have a single network to recognize the human action, and multiple networks for prediction of motion, picked up by a selector, similarly to the idea of MoE. 

% - However, the two problems are partially interconnected;

% - And, it is not clear how to deal with transient phases when human actions alter. 

As we can see, the latest described architecture is similar to the MoE notion, however with some differences. The last architecture is composed of two sets of NNs, first, the human action recognition is learned, and then the output of the action recognition network, as well as input data, are used to learn human motion prediction.
On the other side, in MoE, gate outputs are not directly controlled.
%, and it is a way to increase the sparsity among the experts. 
So, here as shown in Fig.~\ref{fig:MoE:architecture} the two ideas are merged in a single network with two outputs. The gate output predicts the human action, and, expert outputs predict human motion. The gate behavior is guided or controlled via enforcing it to predict human actions and as a result, each expert is trained to learn the motion associated with an action. As we can see in the schematic architecture in the training phase, the gate weights are learned such that they minimize both the error of human action and motion prediction. Moreover, this approach intrinsically allows for smooth transient phases. Finally, the probability distribution of the motion prediction can be written as the marginal probability over the gate outputs, i.e.:
\begin{equation}
    \mathcal{P}(y|X) = \sum_{i=1}^{N}\mathcal{P}(y_i|X, a_i)\mathcal{P}(a_i|X),
    \label{eq:experts-summation}
\end{equation}
where $y$ is the output vector, $X$ is the input vector, $y_i$ is the output of the expert $i$ associated with action $a_i$.

As described in \eqref{eq:recognition-prediction-problem-1} and \eqref{eq:recognition-prediction-problem-1}, the problem of action and motion prediction can be solved in a recursive fashion, i.e., repeat the process for the future time horizon $T$. Another approach is to predict directly for all the future time horizon $T$. This way, we expect to enhance the computational time and be suitable for real-time applications, as it computes the outputs for all the time horizon in the future in a tensor form.
% i.e., with vectorized and matrix operations in parallel, while solving them recursively requires more computational time.
%This way, the proposed approach can be better adapted for real-time scenarios.
\iffalse
Moreover, if decided to solve action and motion prediction problems for the time horizon $T$ directly (avoid using recursive fashion), then for the architecture proposed in \eqref{eq:optimal-state-space-discretized-2}, it is not possible anymore to have selector that choose the predictor associated with the highest probable action since human may change its action in the middle of future time horizon $T$, whereas the probabilistic summation approach allows for it. 
\fi
% To overcome those difficulties, we are presenting an extension of Mixture of Experts idea to simultaneously solve the two problems together.

% Differently from conventional MoE, in this architecture, we have two outputs: 

% - The gate output predicts the human action, and, experts output predict human motion for the given time horizon in the future

% We can write down the network loss function as the sum of the two loss functions related to action recognition and motion prediction; and solve them in a single optimization problem.


% In the literature, these two problems are normally handled separately like a waterfall approach (first classifying and then predicting), however, one can debate their dependency and correlation when more than one step is going to be predicted. Moreover, in the transient phases, when the human is switching from one action to another, the waterfall approach may not effectively resolve the two entangled problems.




% - discuss on how to solve the problem instead of recursive approach, all the future time horizon at the same time --> make discussion that recursive approach is more expensive computationally, hence for real-time applications, maybe directly learning for all the future time horizon can help to run them fast.

% - bring the discussion from the presentations

% - make the discussion that, after the t+1, all the action recognitions depends also on the motion prediction as it goes inside the terms while other design choices does not allow for that, I mean action recognition is independent of the motion prediction.

% - add the probability formulas to the methods' description in the main text.

% - check if to use y or y-hat inside the formulas shown here.

% \section{Proposed Solution Extension}
% \label{sec:appendix:ProposedSolutionExtension}

% \textcolor{blue}{In this appendix, more details related to proposed solution and materials are provided.}


%%%%%%%%%%%%%%%%
